CODAR: A Contextual Duration-Aware Qubit Mapping for Various NISQ Devices

Quantum computing devices in the NISQ era share common features and challenges like limited connectivity between qubits. Since two-qubit gates are allowed on limited qubit pairs, quantum compilers must transform original quantum programs to fit the hardware constraints. Previous works on qubit mapping assume different gates have the same execution duration, which limits them to explore the parallelism from the program. To address this drawback, we propose a Multi-architecture Adaptive Quantum Abstract Machine (maQAM) and a COntext-sensitive and Duration-Aware Remapping algorithm (CODAR). The CODAR remapper is aware of gate duration difference and program context, enabling it to extract more parallelism from programs and speed up the quantum programs by 1.23 in simulation on average in different architectures and maintain the fidelity of circuits when running on Origin Quantum noisy simulator.

==> absmachine.tex <==
\subsection{Abstract Machine}
\label{sec:absmachine}

\input figs/syntax


==> back.tex <==
\section{Background} % and Related Work}
\label{sec:back}
In this section, we first introduce basic concepts of QC,
and then focus on the characteristics of NISQ hardware
which influence the qubit mapping.
%and finally introduce related work.

\subsection{Quantum Computing Basics}
\label{sec:back:qc}
In QC,
information is stored in quantum bits -- \kw{qubits}
and computation is performed by applying quantum gates
and measurements to the quantum state of qubits.
The state of a single qubit $\ket{\psi}$ is a two dimensional complex vector,
\begin{equation}
\small
\ket{\psi}=\alpha\ket{0}+\beta\ket{1}=\alpha\left[
\begin{array}{c}
     0  \\
     1 
\end{array}
\right]+\beta\left[
\begin{array}{c}
     1  \\
     0 
\end{array}
\right]=\left[
\begin{array}{c}
     \alpha  \\
     \beta 
\end{array}
\right]
\label{eq:superposition}
\end{equation}
which is an arbitrary \kw{superposition} of the two basis states %labeled 
($\ket{0}$, % (or $\ket{g}$, ground state) 
$\ket{1}$) %(or $\ket{e}$, excited state)
with complex amplitudes $\alpha,\beta$ %\in\mathbb{C}$
satisfying $|\alpha|^2+|\beta|^2=1$.
%
The number of quantum states grows exponentially 
with the number of qubits in a quantum system.
\iffalse
A general system with $n$ qubits can live in the superposition of $2^n$ basis states, \ie
\begin{equation}
\small
\sum\limits_{\qn{q}\in\{0,1\}^n}c_{\seqn{q}}\ket{\seqn{q}}=\sum\limits_{i=0}^{2^n-1}c_i\ket{i}
\end{equation}
where $\seqn{q}$ is a binary number of integer $i$,
and the complex amplitudes $c_i$ %($i\in[0,2^n-1]$) 
satisfy $\sum\limits_{i=0}^{2^n-1}|c_i|^2=1$.
\fi
This %property 
sets the foundation of potential quantum speedup over classical computation.

\subimport{figs/}{qpic.tex}

Quantum gates operate on qubits and change 
their state.
Fig.~\ref{fig:gates}
lists common single-qubit gates (\eg \kn{H}, \kn{X}, \kn{Y}, \kn{Z}, \kn{S}, \kn{T}) 
and a useful two-qubit gate (\eg \kn{CNOT}).
All of them are reversible~\cite{nielsen2010quantum:qcqi},
%that is,
%each
%such as X,Y,Z,H(Hadamard gate),S(phase gate),T($\pi/8$ gate),Steg,Tteg,UI
and can be described by a %$2\times2$ 
unitary matrix $U$,
%($2\times 2$ for 1-qubit gate, $4\times 4$ for 2-qubit gate)
where $U^{\dagger}U=1$ 
($U^\dagger$ is the adjoint of $U$).
An arbitrary $U$ operator on a %single 
qubit can be written as a combination of rotations, 
together with global phase shifts on the qubit: %~\cite{nielsen2010quantum:qcqi}:
\begin{equation}
\small
    U=e^{i\alpha}R_z(\beta)R_y(\gamma)R_z(\delta) 
\label{eq:ugate}
\end{equation}

The \kn{CNOT} gate operates on 
a {control qubit} $\ket{c}$ and a {target qubit} $\ket{t}$,
performing %the action given by 
$\ket{c}\ket{t}\rightarrow\ket{c}\ket{t\oplus c}$;
%that is, 
if $\ket{c}$ %the control qubit 
is $\ket{1}$ then $\ket{t}$ %the target qubit 
is flipped, otherwise $\ket{t}$ is left alone.
%Multi-qubit gates are very hard to realize in hardware,
%however,
%they may be composed from \kn{CNOT} and single qubit gates~\cite{nielsen2010quantum:qcqi}.
%
Information stored in a qubit is retrieved by the measurement or readout, 
which collapses the state to %one of the basis states (\ket{0} or \ket{1}). %, a classical output.
\ket{0} or \ket{1}.
The outcome is either 0 or 1 with probability $|\alpha|^2$ or $|\beta|^2$, respectively. 

Quantum states are intrinsically delicate~\cite{gottesman2010introQEC}: 
%on the one hand, 
quantum gates may introduce small errors 
which will accumulate; %and eventually become a big error.
and %on the other hand,
looking at one quantum state will collapse it, 
\ie the loss of quantum coherence or decoherence~\cite{zurek1991decoherence}.

\subsection{Characteristics of NISQ Devices}
\label{sec:back:hw}
NISQ devices are expected to have dozens to hundreds of qubits
which have short coherence time, high gate error rates
and limited qubit connectivity~\cite{preskill2018nisq}. 
Due to %limited number of qubits in the NISQ era and 
high overhead of QEC, %~\cite{gottesman2010introQEC},
NISQ systems will not implement error correction. % codes.
Thus logical qubits in the quantum program must 
be mapped into physical qubits following QC device constraints.


\subimport{figs/}{qc-args}
\iffalse
Qubits can be realized on different 
Quantum Information Processing (QIP) platforms,
including superconducting circuits, %~\cite{devoret2013superconducting,reagor2016coherence},
ion trap %~\cite{maslov2017iontrap,lekitsche2017ionQC}
and 
neutral atom. %~\cite{sheng2018PRL121.240501,zeng2017PRL119.160502}.
\fi
To the best of the authors' knowledge,
fully programmable QC devices included 
those built on the superconducting circuits~\cite{devoret2013superconducting,ibmqdevice,reagor2016coherence}
and trapped ions~\cite{debnath2016ionqc,maslov2017iontrap,lekitsche2017ionQC}. %technologies.
%\redt{[TODO]} 
Elementary single- and two-qubit gates based on neutral atom technology
have been developed to lay the foundation for building QC devices~\cite{maller2015rydberg,zeng2017PRL119.160502,sheng2018PRL121.240501}.
%https://web.physics.ucsb.edu/~martinisgroup/
Superconducting circuit 
is currently the most promising technology,
which is being used by 
IBM, Google, Rigetti and Intel;
IonQ, a startup in Maryland, 
is working to build machines based on trapped ions~\cite{debnath2016ionqc,wright2019benchmarking}.

\subimport{figs/}{qcdevices}

%http://iontrap.umd.edu/publications/
Fig.~\ref{fig:qcdevices} shows the 
qubit connectivity graphs (or \kw{coupling maps})
of several programmable QC devices.
The coupling map might be directed graph
like Fig.~\ref{fig:qcdevices} (a) and (b), or undirected like (c),
or fully-connected like (d) and (e).
For the directed graph, %superconducting IBM Q devices,
each arc from physical qubit $p_i$
to $p_j$ indicates that a \kn{CNOT} gate with control qubit $p_i$ and target qubit $p_j$ can be applied.
Although current 5- or 11-qubit trap-ion QC systems~\cite{debnath2016ionqc,wright2019benchmarking} are fully-connected,
it is difficult to maintain full connectivity as the number of qubits grows.
Thus the compiler need do mapping transition
to remap two logical qubits of a two-qubit gate to 
two coupled physical qubits.
This qubit mapping problem has been proved to be NP-complete~\cite{siraichi2018qubitalloc}.

%Recent research on the qubit mapping problem is mainly for superconducting circuits~\cite{siraichi2018qubitalloc,li2019tackling,murali2019noise}.
To perform two-qubit gates between non-adjacent qubits,
additional \kn{SWAP} operations have to be inserted that
exchange the state of two physical adjacent qubits and,
by this, ``moving'' the logical qubits to positions where they can interact with each other.
%until the two of interest for a given \kn{CNOT} computation are in adjacent locations.
As shown in Fig.~\ref{fig:swap},
each \kn{SWAP} operation 
exchanges qubits 
$p_a$ and $p_b$
at the expense of three \kn{CNOT} gates if the connecting edge is bidirectional (Fig.~\ref{fig:swap} (a)),
or three \kn{CNOT} and two levels of \kn{H} gates if undirected (Fig.~\ref{fig:swap} (b)). 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.38\textwidth]{figs/swap.png}
    \caption{The identical transformations for \kn{SWAP}.}
    \label{fig:swap}
\end{figure}

We want to know more about the impact of different quantum technologies on the mapping problem.
Linke \etal made an experimental comparison of 
two 5-qubit leading platforms: 
trapped ions (Ion Q5) and superconducting circuits (IBM Q5)~\cite{linke2017QCcomparison}.
The directly implementable elementary gates in Ion Q5 are
single-qubit gate R$^\theta_\alpha$ 
(rotations by an angle $\theta$ about any axis $\alpha$) 
and two-qubit gate \kn{XX}.
Specifically, 
\kn{CNOT} gate can be implemented by
a one-\kn{XX} and four-\kn{R}~\cite{debnath2016ionqc}.
Linke \etal conclude that
the superconducting system offers faster
gate clock speeds and a solid-state platform, 
while the ion trap system features superior qubits and reconfigurable connections.

Table~\ref{tab:qc-args}
lists parameter information of some QC devices 
based on ion trap, superconducting and 
neutral atomic quantum technologies, respectively.
From the table,
we see that two-qubit gate executes slower 
(at least 2$\times$) 
and has lower fidelity than single-qubit gate
on both superconducting and ion trap platforms;
the ion trap system is about 1000$\times$ slower than 
the superconducting system, 
but can execute more gates before decoherence.
Neutral atoms are %generally 
similar in magnitude to trapped ions.
However, 
the two-qubit gate applied to neutral atoms may not perform slower than a single-qubit gate, 
but the fidelity is much worse. 
%
Moreover,
it has been observed in numerous superconducting architectures that 
the qubit coherence time and fidelity of gates 
can fluctuate unpredictably
%for IBM Q16, $T2$ varies up to 9.2x spatially and temporally across qubits and daily calibrations,
~\cite{murali2019noise}.
These fluctuations are still a challenge~\cite{klimov2018PRL121.090502},
and imply only very short programs can execute reliably on the 
QC devices.

In view of the above, 
we consider the following four major constraints of QC hardware in this paper:
%Neutral atoms provide qubits similar to trapped ions.
\begin{enumerate}[label=\arabic*.]

\item {\bf Qubit Coupling.} 
Each two-qubit gate can only be applied to
two physically nearby qubits connected in some 2D coupling structure.

\item {\bf Qubit Lifetime.}
A qubit retains its %superposition 
state for a very short time. %due to decoherence.
The %state-of-the-art 
coherence time
can reach at most $100\mu s$ for superconducting,
$1s$ for ion trap.
All the computation must be completed within a fraction of qubit coherence time.

\item {\bf Operation Duration.}
Different quantum operations have different execution durations,
and operations applied to disjoint qubits can be performed in parallel.

\item {\bf Operation Fidelity.}
Quantum operations applied to the qubits can introduce errors.
The error rate is unstable and affected by the operation and  physical qubits applied.
Since the qubit becomes fragile over time, 
it introduces less error if we perform operations on it as early as possible.
\end{enumerate}

Therefore, 
it is important to parallelize quantum operations in a quantum program  
and to minimize the longest execution time of all operation sequences in parallel.
%The execution time of a quantum program is determined by 
%the \kw{longest execution path} of quantum operation sequences.


==> evalb.tex <==
\section{Experimental Evaluation}
\label{sec:eval}
In this section, 
we evaluate \mysys with benchmarks based on the latest reported hardware models. 
We compare the runtime of circuits generated by \mysys with the best known algorithm 
to show \mysys's weighted circuit depth reduction effect. 
\subsection{Methodology}
\mysect{Benchmarks}
We totally collect 47 benchmarks which are selected from the previous work including
\begin{itemize}
    \item Programs from IBM Qiskit~\cite{cross2018ibmqiskit}'s github and  RevLib~\cite{wille2008revlib}.
    \item Several quantum algorithms compiled from ScaffCC~\cite{abhari2014scaffcc} and Quipper~\cite{green2013quipper}.
    \item Benchmarks used in the best known algorithm SABRE~\cite{li2019tackling}.
\end{itemize}

\mysect{Hardware Model and Configuration}
\label{sec:eval:config}
We test our algorithm on several hardware models including IBM Q20 Tokyo (Not grid model) shown in Fig.\ref{fig:qcdevices}(c), 
$2 \times 8$ and $6\times6$ grid models shown in Fig.\ref{fig:eval:devices},
where $6\times6$ grid model is
proposed by Enfield~\cite{siraichi2018qubitalloc}'s github. 
The gate duration difference configuration is based on experimental data of symmetric superconducting technology 
shown in Table~\ref{tab:qc-args} 
where two-qubit gate duration is generally twice as much as that of single-qubit gate. 
%We assume \kn{SWAP} operation consists of three \kn{CNOT}s in the test. 
\iffalse
The duration of each kind of gates is listed:
\begin{itemize}
    \item single-qubit gate = 1 cycle
    \item CNOT = 2 cycle
    \item SWAP = 6 cycle
\end{itemize}
\fi

\begin{figure}[htbp]
\centering
%\scriptsize
\footnotesize
\begin{minipage}[b]{.28\textwidth}
\centering
    \includegraphics[width=0.6\textwidth]{figs/2t8arch.JPG}
    \\~~\\~~\\
{(a) $2 \times 8$ gird model}\\
\end{minipage}
\hfill
\begin{minipage}[b]{.13\textwidth}
\centering
    \centering
    \includegraphics[width=0.8\textwidth]{figs/6t6arch.JPG}
    \\
{(b) $6 \times 6$ gird model}
\end{minipage}
\caption{$2 \times 8$ and $6 \times 6$ gird models for evaluation.}
\label{fig:eval:devices} 
\end{figure}

\input{test.tex}

\mysect{Comparison with Previous Algorithms}
There are several recent algorithms that can solve qubit mapping problem proposed by IBM~\cite{qiskit},
Siraichi $\etal$\cite{siraichi2018qubitalloc}, 
Zulehner $\etal$\cite{zulehner2019mapping} and Li $\etal$\cite{li2019tackling}. 
Among them, 
Li's $SABRE$~\cite{li2019tackling} beats the other three in experiment,
thus it is used for comparison in this paper. 
Enfield~\cite{siraichi2018qubitalloc} has rewrote $SABRE's$ algorithm in C++ and 
can output the complete transformed OpenQASM program, 
so we use $SABRE$ implemented by Enfield. % and \mysys to transform several quantum algorithms. 
$SABRE$'s algorithm has a weight parameter $\delta$ for tradeoff between gate number and circuit depth. 
We tune the value of $\delta$ and control $SABRE$ focusing on the circuit depth for the comparison. 

 \begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/initial.png}
    \caption{Method to find a better initial mapping.}
    \label{fig:initmapping} 
 \end{figure}
\iffalse
\bbR{For a fair comparison, \mysys use the same initial mapping as $SABRE's$. We build a simulator which will run the transformed circuits under maximum parallelization and count cycles the circuits use for comparison between $SABRE$ and \mysys. }{}
\fi

\mysect{Initial Mapping}
Initial mapping have been proved to be significant in qubit mapping problem\cite{zulehner2019mapping,siraichi2018qubitalloc}. \kw{Reverse Traversal for Initial Mapping} skill proposed by $SABRE$ is used to generate initial mapping.
This skill first generates a random initial mapping and 
applys SWAP-based heuristic search to traverse through the original gate sequence. 
Then the final mapping obtained by this forward traversal 
is used as initial mapping to apply heuristic search again through the reversed gate sequence. 
The final mapping obtained by this reversed traversal will be used to update the initial mapping for the original circuit. Fig.\ref{fig:initmapping} illustrates the process.\par
For a fair comparison, both \mysys and $SABRE$ use  the same skill to iterate for initial mapping
while the only difference is that they use their own SWAP-based heuristic search respectively in traversal. 
Both \mysys and $SABRE$ iterate 3 times and choose the best initial mapping as final initial mapping. 
For each benchmark, both \mysys and $SABRE$ will randomly generate the first initial mapping 
12 times to iterate for initial mapping and the best one is used for comparison.\par
\iffalse
\bb{We use the $Reverse\ Traversal\ for\ Initial\ Mapping$ method proposed by $SABRE$\cite{li2019tackling} to generate initial mapping. 
In order to make qubits of the the first several two-qubit gates closer, we simply reverse the gate sequence \lgates{} and get \lgates{rev}. Then we use a random initial mapping \qmap{0} and apply \mysys on \lgates{rev} (as round 0) and get a final mapping \qmap{1}. Since no more \kn{SWAP} would be launched at the end, \qmap{1} guarantees at least the last few two-qubit gates launched by round 0 has a very short distance. If we reverse \lgates{rev} back to \lgates{} and use \qmap{1} as the initial mapping, some of the first several two-qubit gates could be executed without remapping. Experiment shows that such initial mapping is not perfect enough. We could apply \mysys on \lgates{} with \qmap{1} as the initial mapping (round 1), and get final mapping \qmap{2}. Similarly can we run \lgates{rev} again and get \qmap{3}. The above process can be illustrated by Fig. \ref{fig:initmapping}. After iteration several rounds(often we choose 10 rounds), we select round $i$ with least total execution time in those rounds. If $i$ is odd, \qmap{i} is the best inital mapping and the output \lgatesschd{i} of round $i$ is the final output. Otherwise, the best initial mapping is \qmap{i + 1} and we reverse \lgatesschd{i} to \lgatesschd{i}' = \{ ($g_j$, $t_j'$) | ($g_j$, $t_j$) $\in$ \lgatesschd{i}, $t_j' = T - t_j - g_j.\tau$ \} as output, where $T$ is the total execution time of round $i$.}
\fi



% For a fair comparison, \mysys use the same skill——$Reverse\ Traversal\ for\ Initial\ Mapping$ proposed by $SABRE$ to generate initial mapping. Both $SABRE$ and \mysys will traverse the program 5 times to decide initial mapping for each benchmark. The minimum depth among 5 iterations will be regarded as the result for that benchmark.

\mysect{Simulator}
There is no simulator considering gate duration difference for quantum program up to now. 
We build a simulator ourselves whose execution way is based on the level compaction idea proposed by \cite{maslov2008quantum}. 
With the largest parallelism, 
the simulator greedily issues gates which has no predecessor and free associate physical qubits. 
The simulator collects the start time of all gates to calculate the circuit's weighted depth.

\subsection{Weighted Circuit Depth Reduction}
Table~\ref{tab:test} shows the weighted circuit depth reduction of \mysys compared with $SABRE$\cite{li2019tackling}. 
\lgate{t} and \lgate{c} respectively denote the total number of gates and the number of \kn{CX} in the original circuit. 
$T_o$ denotes the circuit's original weighted depth without any SWAP inserted. 
$T_C$ and $T_S$ respectively denote the weighted depth of program generated by \mysys and $SABRE$ in three models. 
The comparison between $T_C$ and $T_S$ shows that \mysys can generate program with less weighted depth 
which directly relates to execution time than $SABRE$ for most of benchmarks on different models. 
The benchmark "volumn\_n5\_n2" does not need inserting SWAP 
if the algorithm can find a good initial mapping. 
Both \mysys and $SABRE$ successfully find the ideal initial mapping in three model and 
both $T_C$ and $T_S$ are equal to $T_o$.
%\mysect{Model IBM Q16} 

{\bf Model IBM Q16.} 
On the model IBMQ16, 
the ratio $T_C/T_S$ is 82.5\% at average. 
\mysys successfully beats $SABRE$ for all benchmarks on this model.

%\mysect{Model IBM Q20 Tokyo} 
{\bf Model IBM Q20 Tokyo. } 
On the model IBM Q20 Tokyo, the ratio $T_C/T_S$ is 82.4\% at average. 
\mysys performs not so good on the IBM20 Tokyo compared with those on anothor two models. 
There are few benchmarks (5 in 47) for which \mysys generates circuits with larger weighted depth than $SABRE$. 
The reason for this phenomenon is that IBM Q20 Tokyo is not a grid model and 
the fine priority for heuristic search we discuss in Section~\ref{sec:algorithm}
cannot be used on this platform and the look ahead ability of \mysys is reduced.

%\mysect{Model Enfield 6$\times$6} On the model 
{\bf Model Enfield 6$\times$6} On the model 
IBM Q16, the ratio $T_C/T_S$ is 80.6\% at average.
\mysys perform best in this model and it successfully beat $SABRE$ for all benchmarks.\par
\iffalse
\fi
\iffalse
 . \par

\fi
\iffalse
\bbR{
\mysys performs well on various kind of quantum algorithm benchmarks including Quantum Fourior Transform and so on. It can reduce 17.2\% of the weighted circuit depth at average and halves the depth at best.
}{}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/isingmodel16x1000.png}
    \caption{
        Experience result for trying random initial mapping and apply \mysys and $SABRE$ on ising model 16.
        We selected the hardware as $6 \times 6$ grid model and ran 1000 times for both of the two remapping methods.
        ising model 16 is one of the worst benchmark we found for \mysys compared with $SABRE$.
        both \mysys and $SABRE$ could reach a total execution time of 91 in there best perfect,
        but \mysys may be more fragile facing worse initial mapping in this case.
    }
    \label{fig:isingmodel16x1000}
\end{figure}
\fi
\iffalse
\subsection{Limitation and Future Work}
\mysys still has several limitations. 
The first drawback is that \mysys's heuristic search function is not perfect now 
and perform not so well in not grid model (IBMQ20 Tokyo) compared to its good performance in grid model (IBMQ16 and Enfield 6$\times$6). 
The look ahead ability of \mysys in not grid model is not perfect and will generate several worse program for some benchmarks (7 in all 168 cases). \mysys is greatly affected by initial mapping in some cases, e.g. ising model 16(Fig. \ref{fig:isingmodel16x1000}). We will focus on improve the heuristic search algorithm in the future work.
\fi







==> figs/ex-qft4-1.tex <==
\begin{figure}[h]
\begin{minipage}[b]{.12\textwidth}
\centering
{
\includegraphics[width=0.65\textwidth]{figs/grid4.png}
\\~~\\~~
{(a)}
}
\end{minipage}
\iffalse
\begin{minipage}[b]{.35\textwidth}
\centering
\scriptsize
\begin{tabular}{c|c|c|c}
\hline
    Gate  & T & CX & SWAP 
    \\
    \hline
    Duration & 1 cycle &2 cycle & 6 cycle
    \\
    \hline
\end{tabular}
\\~~\\
%\qquad
\includegraphics[width=0.5\textwidth]{figs/ex-qft4-1.png}
\\~~
\normalsize
{(b)}

\end{minipage}
\fi
~
\begin{minipage}[b]{.35\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/ex-qft4-1a.png}
\\~~
{(c)}
\end{minipage}
\\ \\
\begin{minipage}[b]{.12\textwidth}
\centering
\scriptsize
\begin{tabular}{c|c}
\hline
    Gate  & Duration
    \\
    \hline
    T & 1 cycle \\
    \hline
    CX & 2 cycle \\
    \hline
    SWAP & 6 cycle \\
    \hline
\end{tabular}
\\ ~ \\
%\qquad
\includegraphics[width=1\textwidth]{figs/ex-qft4-1.png}
\\~~
\normalsize
{(b)}
\end{minipage}
~
\begin{minipage}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/ex-qft4-1b.png}
\\
{(d)}
\end{minipage}
\caption{An example reflecting the impact of {\bf program context} on SWAP-based transformations: 
%: (a) qubits coupling map and gate durations, (b) OpenQASM code fragment,
\kn{SWAP q[3], q[1]} is selected in (d) to avoid using \kn{q[2]} operated by the previous \kn{T} gate, accordingly increasing parallelism.}
\label{fig:ex1:qft4}
\end{figure}


==> figs/ex-qft4-2.tex <==
\begin{figure}[h]
\begin{minipage}[b]{.15\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{figs/grid4.png}
\\
{(a)}
\end{minipage}
\begin{minipage}[b]{.35\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figs/ex-qft4-2a.png}
\\
{(c)}
\end{minipage}
\\~~\\
\begin{minipage}[b]{0.15\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figs/ex-qft4-2.png}
{(b)}
\end{minipage}
~
\begin{minipage}[b]{0.35\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figs/ex-qft4-2b.png}
\\{(d)}
\end{minipage}
\caption{A 4-qubit QFT example reflecting the impact of {\bf gate duration difference}: 
``\kn{SWAP q[3],q[1]}'' 
is the best candidate
since it can start immediately after
``\kn{T q[1]}'' while ``\kn{CX q[0],q[2]}'' has not finished yet, increasing the parallelism of the circuit.}
\label{fig:exdu:qft4}
\end{figure}


==> figs/gatecommutativity.tex <==
\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \hline
         & H & X & Y & Z & Rz & CX.C & CX.T \\
         \hline
       H & 1 & 0 & 1 & 0 & 0 & 0 & 0 \\
       \hline
       X & 0 & 1 & 1 & 1 & 0 & 0 & 1\\
       \hline
       Y & 1 & 1 & 1 & 1 & 0 & 0 & 0\\
       \hline
       Z & 0 & 1 & 1 & 1 & 1 & 1 & 0\\
       \hline
       Rz & 0 & 0 & 0 & 1 & 1 & 1 & 0\\
       \hline
       CX.C & 0 & 0 & 0 & 1 & 1 & 1 & 0 \\
       \hline
       CX.T & 0 & 1 & 0 & 0 & 0 & 0 & 1\\
       \hline
    \end{tabular}
    \caption{Commutativity table between quantum operations. The table is diagonally symmetric. 
    Each head of the table represents a kind of gate on a specific qubit. 
    \kn{CX.C}, \kn{CX.T} represent using the qubit as the control or target qubit of \kn{CX}. 
    If the cell in row $a$ and column $b$ is 1, it means operation $a$ commutes with $b$. 
    For example, the cell in row \kn{X} and column \kn{CX.T} is 1, 
    which means that applying \kn{X} gate on a specific qubit \lqubit{} commutes with a \kn{CX} gate which uses \lqubit{} as target qubit. 
    %the item in "X" row and \kn{"CX.C"} column is 0 which means that applying X gate on a specific qubit $q$ does not commute with a CNOT gate which uses q as control qubit.
    The \kn{Rz($\theta$)} gate is a single-qubit rotation through angle $\theta$ (radians) around the z-axis, 
    and it is the same as gate \kn{U1}$(\theta)$. 
    \kn{T} = \kn{Rz}$(\pi / 4)$ and \kn{S} = \kn{Rz}$(\pi / 2)$,
    which are the special cases of \kn{Rz}.
    }
    \label{tab:commutativity}
\end{table}


==> figs/qcdevices.tex <==
\begin{figure}[htbp]
\centering
\scriptsize
\begin{minipage}[b]{.1\textwidth}
\centering
  \includegraphics[width=\textwidth]{devices/ibm-qx4-tenerife.png}
{(a) IBM QX4}
\end{minipage}
\hfill
\begin{minipage}[b]{.36\textwidth}
\centering
  \includegraphics[width=\textwidth]{devices/ibm16-melbourne.png}
\\
~~\\
{(b) IBM Q16 Melbourne}
\end{minipage}
\hfill
\begin{minipage}[b]{.15\textwidth}
\centering
  \includegraphics[width=\textwidth]{devices/ibm-q20.jpg}
{(c) IBM Q20}
\end{minipage}
\hfill
\begin{minipage}[b]{.1\textwidth}
\centering
  \includegraphics[width=\textwidth]{devices/ionqc5.png}
\\
~~\\
{(d) Ion Q5~\cite{debnath2016ionqc}}
\end{minipage}
\hfill
\begin{minipage}[b]{.12\textwidth}
\centering
  \includegraphics[width=\textwidth]{devices/ionqc11.png}
\\
~~\\
{(e) Ion Q11~\cite{wright2019benchmarking}}
\end{minipage}
\caption{Coupling maps of some QC devices.} %IBM Experience Q devices~\cite{ibmqdevice} and 5-qubit Ion quantum computer~\cite{debnath2016ionqc}}
\label{fig:qcdevices}
\end{figure}


==> figs/qpic.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{tikz}
%\usepackage{braket}
%\usepackage{varwidth}
%\usepackage[braket]{qcircuit}
%\usepackage{graphicx} 
%\usepackage{amsmath}
%\usepackage{subfigure}
%\usepackage{subcaption}
%\usetikzlibrary{calc}
%\usetikzlibrary{backgrounds}
%\usetikzlibrary{math}
%\begin{document}

\begin{figure}[htbp]
\centering{
%\footnotesize{
\scriptsize{
\begin{minipage}[c]{.22\textwidth}
\centering  
%\scalebox{0.8}{
$$
\begin{array}{rcl}
  %  name & logo & matrix \\
  % \hline
%\vspace{0.5em}
\tt{Hardmard} &
\subimport{qpic/}{H.tikz} &
%$${
           \dfrac{1}{\sqrt 2}
           \begin{bmatrix}
           1 & 1	\\
           1 & -1  \\
           \end{bmatrix}
%}$$ 
\\
\vspace{0.5em}
\tt{Pauli-X} &
\input{qpic/X.tikz} &
%$${
    \begin{bmatrix}
    0 & 1	\\
    1 & 0
    \end{bmatrix}
%}$$ 
\\
\vspace{0.5em}
\tt{Pauli-Y} &
\subimport{qpic/}{Y.tikz} &
%$${
    \begin{bmatrix}
    0 & -i	\\
    i & 0
    \end{bmatrix}
%}$$ 
\end{array}
$$
\end{minipage}
\hfill
\begin{minipage}[c]{.22\textwidth}
%\vspace{0.5em}
$$
\begin{array}{rcl}
\tt{Pauli-Z} &
\subimport{qpic/}{Z.tikz} &
%$${
    \begin{bmatrix}
    1 & 0	\\
    0 & -1
    \end{bmatrix}
%}$$ 
\\
\vspace{0.5em}
\tt{Phase}   &
\subimport{qpic/}{S.tikz} &
%$${
    \begin{bmatrix}
    1 & 0  	\\
    0 & i  	\\
    \end{bmatrix}
%}$$ 
\\
%\vspace{0.5em}
\pi/8 &
\subimport{qpic/}{T.tikz} &
%$${
    \begin{bmatrix}
    1 & 0  	\\
    0 & e^{i\pi/4}  	\\
    \end{bmatrix}
%}$$  
\end{array}
$$
%\subcaption{(a) Single qubit gates}
\label{fig:C:qpic1}
\end{minipage}
%\hfill
\begin{minipage}[c]{.44\textwidth}
%\vspace{0.5em}
$$
\begin{array}{lrl}
\cell{
~~controlled-NOT (\tt{CNOT}) \\
~~or controlled-X (\tt{CX})
%\vspace{0.5em}
\\
%\vspace{1em}
}
&
\cell{
\subimport{qpic/}{CNOT.tikz}\\
}
&
{
U_{CN}=
\begin{bmatrix}
1 & 0 & 0 & 0 	\\
0 & 1 & 0 & 0 	\\
0 & 0 & 0 & 1 	\\
0 & 0 & 1 & 0 	\\
\end{bmatrix}
}
\end{array}
$$
%~~\\
%\centering
%\subcaption{(b) 2-qubit gate: CNOT/CX}
\end{minipage}
}}
\caption{Some common gates: symbols and unitary matrices.}
\label{fig:gates}
\end{figure}


==> figs/syntax.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
\footnotesize
%\scriptsize
$$\begin{array}{@{\,}r@{\ }c@{\ \ }c@{\ \ }l@{\,}}
(\Comm{World})       & \World       & ::= & 
	(\Code, \QArch)  
\\
(\Comm{QuantumArchitecture}) & \QArch   & ::= & 
	(\NQ, \MX, \MY, \PhQubits, \QEdges)  
\\
(\Comm{PhysicalQubits}) & \PhQubits  & ::= & 
	\{\Lq \CAPmapsto (\Lx, \Ly, \ERdout)\}^*  
\\
(\Comm{QubitEdges}) & \QEdges  & ::= & 
	\{\QEdge{\Lq_1}{\Lq_2}{\ECnot}\}^*  
\\
(\Comm{Address})     & \Lq, \Lx, \Ly & \in & 
	\Nat~(\Comm{nat nums}, \Lq\in[0,\NQ), \Lx\in[0,\MX), \Ly\in[0,\MY)) \smallskip
\\
(\Comm{ErrorRate}) & \ERdout,\ECnot  & \in & 
	[0, 1)~(\Comm{scientific form}, \eg $2e-2$)
\\

(\Comm{SingleQubitGate})  & \Sgate        & ::= & 
	\GX \mid \GY \mid \GZ \mid \GI \mid \GH \mid \GS \mid \GT \smallskip
\\
(\Comm{Instr})       & \Instr        & ::= & 
	\Sgate~q \mid \GCN~q_c,q \mid \Rdout~q, c
\\
(\Comm{Qubit})       & q        & \in & 
	\Nat \cup \Qregs
\\
(\Comm{Bit})       & c        & \in & 
	\Nat \cup \Real \cup \Cregs
\\
(\Comm{QubitRegister})     & \Regs         & \in & \Comm{Register} \Arrow \Comm{Word} \smallskip                                  \\
%    (\Comm{SingleQubitGateWithAngle})  & \SAgate    & ::= & \GRx \mid \GRy \mid \GRz \mid \GPh \smallskip				\\
~~\\
(\Comm{LogicQubits})    & \Qubit   & ::= & \qubit \smallskip
						\\
    (\Comm{PhysicalQubits})  & \PQubit   & ::= & i~(\Comm{nat nums}) \smallskip
						\\
    (\Comm{CodeHeap})    & \Code         & ::= & \{\Lf \CAPmapsto \Instr\}^* \smallskip                                         \\
    (\Comm{Qubit})     & \Qubit           & ::= & \Rr_0 \mid \ldots \mid \Rr_{31} \smallskip                                      \\

-------\\

    (\Comm{ThreadState}) & \State        & ::= & (\Mem, \Thread)\smallskip                                                      \\
    (\Comm{Memory})      & \Mem,\Rheap,\Wheap  & \in & \Comm{Address} \Parrow \Comm{Word} \smallskip                                  \\
    (\Comm{Thread})      & \Thread_i     & ::= & (\Regs, \Pc, \Xstate) \smallskip                                               \\
    (\Comm{Address})     & \Lf, \Ll, \Pc & ::= & i~(\Comm{nat nums}) \smallskip                                                 \\
    (\Comm{Word})        & \Word         & ::= & i~(\Comm{nat nums}) \smallskip                                                 \\
    (\Comm{Xstate})      & \Xstate       & ::= & \varepsilon \mid (\Rheap, \Wheap, \Bstate, \Status) \smallskip                 \\
    (\Comm{Bstate})      & \Bstate       & ::= & (\Regs, \Pc) \smallskip                                                        \\
    (\Comm{Status})      & \Status       & ::= & \Active \mid \Commit \mid \Abort \smallskip                                    \\
                         &               & \hfill \mid & \Insn{lw}~\Rrd, \Word(\Rrs) \mid \Insn{sw}~\Rrd, \Word(\Rrs)           \\
                         &               & \hfill \mid & \Insn{cas}_t~\Rrd, \Rrt, \Word(\Rrs) \mid \Insn{out}~\Rrd              \\
                         &               & \hfill \mid & \Insn{beq}~\Rrs, \Rrt, \Lf   \mid \Insn{bne}~\Rrs, \Rrt, \Lf           \\
                         &               & \hfill \mid & \Insn{lw}_t~\Rrd, \Word(\Rrs)\mid \Insn{sw}_t~\Rrd, \Word(\Rrs)        \\
                         &               & \hfill \mid & \Insn{begin} \mid \Insn{validate}~\Rrd \mid \Insn{commit}              \\
    (\Comm{InstrSeq})    & \Iseq         & ::= & \Instr; \Iseq \mid \Insn{j}~\Lf \mid \Insn{jr}~\Rrs                            \\
                         &               & \hfill \mid & \Insn{rollback}                                                        \\
   \end{array}$$
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DISPLAYMATH %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \hrule
  \caption{Syntax of Machine}\label{syntax}
  \end{figure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> model-others.tex <==
\subsection{Machine Models in other Papers}
\label{sec:model:others}
\subsubsection{ASPLOS 2019~\cite{murali2019noise}}
\cite{murali2019noise} uses IBMQ16 (2$\times$8)
Let $Q_P$ be the set of program qubits. 
Let $Q_H$ be the set of hardware qubits. 
In this work, we assume hardware qubits
are arranged as a 2-D grid of dimensions $M_x\times M_y$. 
Likewise,
due to the connectivity characteristics of IBMQ16, 
we assume only hardware qubits which are adjacent in the grid are 
permitted to participate in two qubit operations. 

For $q\in Q_P$, the ordered pair $(q.x, q.y)$ corresponds to
the location of the hardware qubit assigned to the program
qubit $q$. 
Let $G$ be the set of operations in the program. 
This includes single-qubit gates such as \kn{H}, 
and the 2-qubit \kn{CNOT}
gate and qubit measurement or Readout operations. 
\kn{CNOT} and readout operations dominate the reliability outcomes,
so the reliability score focuses on them. 
The subset of \kn{CNOT} gates is denoted by $G_{\kn{CNOT}}$ , 
and the subset of readout operations is $G_{\kn{Readout}}$. 
For each gate $g$ in the program, 
the start time is denoted by $(g.\tau)$, duration by $(g.\delta)$, 
and reliability by $(g.\epsilon)$. 
To denote data dependencies between the operations,
we use a binary relation $>$ on the gates, 
so that for two operations $g_2 > g_1$ if $g_2$ depends on $g_1$ . 
Although the reliability objective focuses on a subset of operations, 
we map and schedule all operations (including single-qubit operations)
to provide a valid real-system executable.

\subsection{QVM}
\href{https://github.com/rigetti/qvm}{QVM}~\cite{smith2016quil}



 


==> related.tex <==
\section{Related Work}
\label{sec:rel}
%\paragraph{Qubit Mapping}
Some recent works~\cite{siraichi2018qubitalloc,zulehner2019mapping,li2019tackling,wille2019mapping,zulehner2019compiling} are proposed for IBM QX architectures %and can handle devices with arbitrary coupling.
\cite{siraichi2018qubitalloc} can only map the logical qubits of small circuits for 5-qubit IBM QX2 architectures. 
%based on only qubit topology information, not calibration data.
\cite{wille2017IBM50} considers all possible applications of the SWAP and H operations that may solve the qubit mapping problem for a given QC circuit which is a computationally task. They utilize powerful reasoning engines as solver to cope with the complexity. Their method can bring at least close-to-minimal result but cannot afford large scale program.\par
\cite{zulehner2019mapping,li2019tackling} use heuristic search to provide good solutions for mapping problem in acceptable time and can be applied to large scale program. 
\cite{zulehner2019mapping} provides a dedicated method for compiling SU(4) quantum circuits to IBM QX architectures. It partition the circuit into layers and focus on finding efficient remapping for each layer. To minimize circuit depth,
\cite{li2019tackling} provide a heuristic search scheme with high efficiency and reduced search space. They use the total distance of all logically executable CNOT as the score for heuristic searching but ignores single qubit gate. Both of them ignore the program context and the gate duration difference which limits them to find remapping solution with better parallelism that shorten the execution time.\par
\cite{shi2019optimized} focus on optimizing compilation of aggregated instruction and propose commutation group data structure for commutativity detection. Similar to us, they use commutativity to extract more parallelism. Their method for commutativity detection has some difference with ours. Their detection focus on finding maximum number of logical executable gates which are not conflict with each other. The commutativity detection in this paper focus on finding all the logical executable gates for a better heuristic search.


%http://cuda.dcc.ufmg.br/enfield/
%https://ysiraichi.github.io/enfield/
%\cite{zulehner2018mapping} 

\cite{zulehner2019compiling} 

==> test.tex <==
\begin{table*}[htbp]
\centering
%\footnotesize
%\normalsize
\begin{tabular}{*{13}{|@{}c}|}
\hline
  \multirow{2}{*}{\textbf{Benchmark}}&\multirow{2}{*}{\textbf{Qubits}} &\multirow{2}{*}{$g_t$} 
  &  \multirow{2}{*}{$T_o$}&\multicolumn{3}{c|}{IBM Q16}  & \multicolumn{3}{c|}{IBM Q20 Tokyo}  &\multicolumn{3}{c|}{Enfield 6*6} \\
\cline{5-13}
 &  &  &  & $T_C$ & $T_S$ &  $T_C/T_S$ & $T_C$ & $T_S$ &  $T_C/T_S$ & $T_C$ & $T_S$ &  $T_C/T_S$ \\ 
\hline
\hline
bv\_n6 & 6 & 17 & 13 & 16 & 29 & 55.2\% & 14 & 17 & 82.4\% & 16 & 23 & 69.6\% \\
\hline
bv\_n8 & 8 & 23 & 17 & 26 & 45 & 57.8\% & 17 & 23 & 73.9\% & 18 & 35 & 51.4\% \\
\hline
bv\_n10 & 10 & 29 & 21 & 29 & 61 & 47.5\% & 21 & 31 & 67.7\% & 26 & 41 & 63.4\% \\
\hline
bv\_n12 & 12 & 35 & 25 & 38 & 73 & 52.1\% & 25 & 41 & 61.0\% & 29 & 59 & 49.2\% \\
\hline
bv\_n14 & 14 & 41 & 29 & 44 & 69 & 63.8\% & 29 & 49 & 59.2\% & 34 & 69 & 49.3\% \\
\hline
bv\_n16 & 16 & 47 & 33 & 51 & 99 & 51.5\% & 36 & 59 & 61.0\% & 38 & 99 & 38.4\% \\
\hline
qft\_n6 & 6 & 81 & 55 & 73 & 103 & 70.9\% & 63 & 97 & 65.0\% & 70 & 97 & 72.2\% \\
\hline
qft\_n8 & 8 & 148 & 79 & 121 & 157 & 77.1\% & 108 & 163 & 66.3\% & 119 & 121 & 98.4\% \\
\hline
qft\_n10 & 10 & 235 & 103 & 171 & 223 & 76.7\% & 161 & 241 & 66.8\% & 168 & 193 & 87.1\% \\
\hline
qft\_n12 & 12 & 342 & 127 & 215 & 283 & 76.0\% & 216 & 343 & 63.0\% & 221 & 355 & 62.3\% \\
\hline
qft\_n14 & 14 & 469 & 151 & 307 & 319 & 96.2\% & 267 & 373 & 71.6\% & 294 & 373 & 78.8\% \\
\hline
qft\_n16 & 16 & 616 & 175 & 370 & 409 & 90.5\% & 327 & 577 & 56.7\% & 364 & 511 & 71.2\% \\
\hline
volume\_n12\_d10\_i0 & 12 & 600 & 100 & 237 & 261 & 90.8\% & 184 & 254 & 72.4\% & 221 & 270 & 81.9\% \\
\hline
volume\_n12\_d20\_i0 & 12 & 1200 & 200 & 507 & 637 & 79.6\% & 410 & 505 & 81.2\% & 495 & 637 & 77.7\% \\
\hline
volume\_n12\_d32\_i0 & 12 & 1920 & 320 & 855 & 1061 & 80.6\% & 668 & 985 & 67.8\% & 828 & 1025 & 80.8\% \\
\hline
volume\_n12\_d3\_i0 & 12 & 180 & 30 & 36 & 42 & 85.7\% & 41 & 46 & 89.1\% & 42 & 51 & 82.4\% \\
\hline
volume\_n12\_d5\_i0 & 12 & 300 & 50 & 104 & 115 & 90.4\% & 85 & 122 & 69.7\% & 93 & 119 & 78.2\% \\
\hline
volume\_n12\_d8\_i0 & 12 & 480 & 80 & 160 & 182 & 87.9\% & 141 & 185 & 76.2\% & 174 & 191 & 91.1\% \\
\hline
volume\_n16\_d10\_i0 & 16 & 800 & 100 & 281 & 352 & 79.8\% & 199 & 299 & 66.6\% & 266 & 291 & 91.4\% \\
\hline
volume\_n16\_d15\_i0 & 16 & 1200 & 150 & 454 & 593 & 76.6\% & 330 & 566 & 58.3\% & 436 & 527 & 82.7\% \\
\hline
volume\_n16\_d20\_i0 & 16 & 1600 & 200 & 634 & 875 & 72.5\% & 467 & 710 & 65.8\% & 577 & 895 & 64.5\% \\
\hline
volume\_n16\_d3\_i0 & 16 & 240 & 30 & 60 & 63 & 95.2\% & 48 & 52 & 92.3\% & 56 & 80 & 70.0\% \\
\hline
volume\_n16\_d5\_i0 & 16 & 400 & 50 & 124 & 174 & 71.3\% & 96 & 172 & 55.8\% & 120 & 127 & 94.5\% \\
\hline
volume\_n16\_d8\_i0 & 16 & 640 & 80 & 241 & 256 & 94.1\% & 162 & 245 & 66.1\% & 190 & 274 & 69.3\% \\
\hline
volume\_n5\_d10\_i0 & 5 & 200 & 100 & 136 & 166 & 81.9\% & 125 & 164 & 76.2\% & 136 & 146 & 93.2\% \\
\hline
volume\_n5\_d15\_i0 & 5 & 300 & 150 & 200 & 293 & 68.3\% & 193 & 200 & 96.5\% & 195 & 228 & 85.5\% \\
\hline
volume\_n5\_d20\_i0 & 5 & 400 & 200 & 252 & 296 & 85.1\% & 242 & 236 & 102.5\% & 252 & 302 & 83.4\% \\
\hline
volume\_n5\_d2 & 5 & 40 & 20 & 20 & 20 & 100.0\% & 20 & 20 & 100.0\% & 20 & 20 & 100.0\% \\
\hline
4mod5-v1\_22 & 5 & 21 & 22 & 42 & 53 & 79.2\% & 22 & 22 & 100.0\% & 42 & 47 & 89.4\% \\
\hline
9symml\_195 & 11 & 34881 & 32084 & 74352 & 81711 & 91.0\% & 59755 & 60884 & 98.2\% & 71816 & 78153 & 91.9\% \\
\hline
adr4\_197 & 13 & 3439 & 3088 & 6977 & 7737 & 90.2\% & 5345 & 5444 & 98.2\% & 6747 & 7479 & 90.2\% \\
\hline
alu-v0\_27 & 5 & 36 & 35 & 61 & 71 & 85.9\% & 49 & 39 & 125.6\% & 68 & 71 & 95.8\% \\
\hline
cycle10\_2\_110 & 12 & 6050 & 5662 & 12871 & 14113 & 91.2\% & 10077 & 10626 & 94.8\% & 12492 & 13682 & 91.3\% \\
\hline
ising\_model\_10 & 10 & 480 & 90 & 89 & 90 & 98.9\% & 89 & 90 & 98.9\% & 89 & 90 & 98.9\% \\
\hline
ising\_model\_13 & 13 & 633 & 91 & 91 & 91 & 100.0\% & 91 & 91 & 100.0\% & 91 & 178 & 51.1\% \\
\hline
ising\_model\_16 & 16 & 786 & 91 & 91 & 91 & 100.0\% & 91 & 180 & 50.6\% & 91 & 130 & 70.0\% \\
\hline
misex1\_241 & 15 & 4813 & 4473 & 9816 & 10775 & 91.1\% & 7196 & 6940 & 103.7\% & 9296 & 10663 & 87.2\% \\
\hline
mod5mils\_65 & 5 & 35 & 37 & 76 & 80 & 95.0\% & 63 & 59 & 106.8\% & 76 & 80 & 95.0\% \\
\hline
radd\_250 & 13 & 3213 & 2990 & 6727 & 7404 & 90.9\% & 5061 & 5375 & 94.2\% & 6494 & 7159 & 90.7\% \\
\hline
rd73\_252 & 10 & 5321 & 4829 & 10970 & 12287 & 89.3\% & 8834 & 8933 & 98.9\% & 10694 & 11780 & 90.8\% \\
\hline
rd84\_142 & 15 & 343 & 191 & 452 & 493 & 91.7\% & 378 & 412 & 91.8\% & 459 & 463 & 99.1\% \\
\hline
rd84\_253 & 12 & 13658 & 12176 & 28256 & 31365 & 90.1\% & 22054 & 23183 & 95.1\% & 27237 & 30133 & 90.4\% \\
\hline
sqn\_258 & 10 & 10223 & 9176 & 20916 & 23170 & 90.3\% & 16741 & 16694 & 100.3\% & 20581 & 22263 & 92.4\% \\
\hline
square\_root\_7 & 15 & 7630 & 6367 & 12399 & 16269 & 76.2\% & 10247 & 10710 & 95.7\% & 12058 & 15744 & 76.6\% \\
\hline
sym6\_145 & 7 & 3888 & 3686 & 8129 & 9011 & 90.2\% & 5885 & 6221 & 94.6\% & 8066 & 8847 & 91.2\% \\
\hline
sym9\_193 & 11 & 34881 & 32084 & 74352 & 81711 & 91.0\% & 59805 & 60777 & 98.4\% & 71920 & 78153 & 92.0\% \\
\hline
z4\_268 & 11 & 3073 & 2756 & 6248 & 6892 & 90.7\% & 5010 & 5140 & 97.5\% & 6082 & 6827 & 89.1\% \\
\hline


\end{tabular}
\iffalse\fi
\begin{tablenotes}
\normalsize
\item \textbf{Qubits}: The number of qubits used in the benchmark. \textbf{$g_t$}: Total number of gates in the original program. \textbf{$T_o$}: Circuit's original weighted depth without any SWAP inserted. \textbf{$T_C$}, \textbf{$T_S$}: Weighted depth of program generated by \mysys and $SABRE$ respectively.
\end{tablenotes}

\caption{Weighted Circuit Depth Compared with SABRE in Different Platform.}
\label{tab:test}


\end{table*}
